Computing Agents for Decision Support Systems

In decision support systems, it is essential to get a candidate solution fast, even if it means resorting to an approximation. This constraint introduces a scalability requirement with regard to the kind of heuristics which can be used in such systems. As execution time is bounded, these algorithms need to give better results and scale up with additional computing resources instead of additional time. In this paper, we show how multi-agent systems can fulfil these requirements. We recall as an example the concept of Evolutionary Multi-Agent Systems, which combine evolutionary and agent computing paradigms. We describe several possible implementations and present experimental results demonstrating how additional resources improve the efficiency of such systems.

==> model.tex <==
%\newcommand\M{\mathcal{M}}
%\newcommand\ID{\mathit{ID}}
%\newcommand\id{\mathit{id}}
%\newcommand\TP{\mathit{TP}}
%\newcommand\tp{\mathit{tp}}

\subsection{Computing MAS model}
\label{model}

The model defines an agent as a tuple:
\begin{equation}
AG \ni ag=\tuple{\id,\tp,dat_1,\ldots,dat_n}
\label{eq:agent}
\end{equation}
where:
\begin{description}  
\item[$\id\in\ID$] is a unique identifier of an agent\footnote{For each
    element of the model its domain, which is a finite set of possible
    values, is denoted by the same symbolic name in upper case, e.g.\ $\ID$
    is the set of all possible agent identifiers.},
\item[$\tp\in\TP$] denotes the type of an agent, depending on its type, an
  agent is equipped with specific data and may perform specific actions,
\item[$dat_i \in DAT_i, i=1,\ldots,n$] represents problem-dependent data
  (knowledge) gathered by an agent (solutions, resources, outcomes of the
  observations etc.).
\end{description}
Since for a particular agent, its identifier and type do not change during
its lifetime, the state of an agent is described by its data (knowledge),
and the state space of an agent may be described as:
\begin{equation}
  X_{AG}=DAT_1\times\cdots\times DAT_N
  \label{eq:ag_state}
\end{equation}

According to \cite{my:HoloMAS2009} a multi-agent system includes agents,
actions to be executed by the agents, available algorithms, and the
environment represented by some common data, which may acquired by the
agents:
\begin{equation}
AS \ni as=\tuple{Ag,Act,Alg,qr_1,\ldots,qr_m}
\label{eq:mas}
\end{equation}
where:
\begin{description}
\item[$Ag \subset AG$] is the set of agents of $as$,
\item[$Act \subset ACT$] describes actions that may be performed by the
  agents of $as$,
\item[$Alg \subset ALG$] is the set of algorithms available in $as$, 
\item[$qr_i \in QR_i, i=1,\ldots,m$] denote queries providing data
  (knowledge) available for all agents in the environment.
\end{description}
For a particular agent system, its actions and algorithms do not change in
time, and its state is determined by the set of agents present in the
system. Thus the state space of a computational system consisting of a
single agent system is:
\begin{equation}
  X=X_{AS}=2^{AG}
  \label{eq:ag_state2}
\end{equation}
The values of queries $qr_i$ do not need to be included in the description
of the system state since they may be treated as (possibly
stochastic\footnote{$\M(A)$ denotes the space of probabilistic measures
  over the measurable set $A$}) functions of the system state:
\begin{equation}
  \lambda_i: X \rightarrow \M(QR_i)
  \label{eq:query_fun}
\end{equation}
For example, there may exists a query that serves for random choosing one
of the agents present in $Ag$.

In the space of types, a subsumption relation $\preceq$ is defined,
which is used to state whether one type is the specialisation of another:
\begin{equation}
  \text{``$\preceq$''} \; \subset \; TP \times TP
\label{eq:subsumption}
\end{equation}
Relation $\preceq$ defines a partial order in $TP$, and $A \preceq B:
A,B\in \TP$ means that $A$ is a subtype of $B$. Since the type of an agent
determines its features, it is assumed that an agent with a more specific
type is able to provide all data and perform all actions of an agent with a
more general type, yet of course the realisation of the descendant may be
different than the parent \citep{my:ICCS2009}.

Agents may perform actions in order to change the state of the system.
An action is defined as the following tuple:
\begin{equation}
ACT \ni act=\tuple{tp, pre, post}
\end{equation}
% where $\tp\in\TP$ denotes the type of agents allowed to execute the action
% (only agents of the type $\tp$ and descendant types -- according to the
% ``$\preceq$'' relation -- may perform the action); $pre\in X$ is the state
% of the system which allows for performing action $act$; $post\in X\times X$
% is the relation between the state of the system before and after performing
% action $act$.
where:
\begin{description}
\item[$tp \in TP$] denotes the type of agents allowed to execute the action
  (only agents of the type $tp$ and descendant types -- according to
  ``$\preceq$'' relation -- may perform the action),
\item[$pre\subseteq X$] is the state of the system which allows to perform
  action $act$,
\item[$post\subseteq X\times X$] is the relation between the state of the system
  before and after performing action $act$.
\end{description}
The descendant types (according to $\preceq$ relation) must hold the
preconditions and postconditions of the parents, yet they may extend these
conditions by adding new alternatives in preconditions and conjunctions in
postconditions. When mentioned conditions are met, the descendant types are
fully substitutable for parent types (in the means of contract
substitutability \citep{meyer}).

% Actions may depend on algorithms, i.e.\ in order to perform an action, one
% or more algorithms may be needed, which is described by the relation:
% \begin{equation}
%   \text{``$\leadsto$''} \subset ACT \times ALG
% \end{equation}
% For algorithms there is also a subsumption relation ``$\preceq$'' defined,
% which states whether one algorithm is a specialization of another:
% \begin{equation}
%   \text{``$\preceq$''} \subset ALG \times ALG
% \end{equation}
% Relation ``$\preceq$'' introduces a partial order in $ALG$, which means
% that if $A_1\preceq A: A_1,A\in ALG$ then $A_1$ can be used in place of $A$
% when needed.

% Further dependencies between algorithms used in the system may be described
% using the following relation:
% \begin{equation}
% \text{``$\leadsto$''} \subset ALG \times ALG
% \end{equation}
% If algorithm $A$ depends on algorithm $B$ ($A \leadsto B$) it means that
% $B$ (or its subtype) is needed for $A$ to function properly.  
% When an action is about to be performed, a subset of algorithms is selected
% from $Alg$ according to $\preceq$ and $\leadsto$ relations. These
% algorithms are said to be ``available'' in the environment for the
% execution of a particular action.

% The proposed formalism allows to formulate the conditions of
% \emph{functional integrity} \citep{my:HoloMAS2009} of agent system
% $as=\tuple{Ag,Act,Alg,qr_1,\ldots,qr_m}$:
% \begin{gather}
% \forall\, act\in Act \, [\,(\exists\, alg\in ALG: act\leadsto alg) \Rightarrow
%  (\exists\, alg_c \in Alg: alg_c \preceq alg)\,]
% \label{eq:integrityAct}\\
% \forall\, alg_1\in Alg \, [\,(\exists\, alg_2\in ALG: alg_1 \leadsto alg_2)
%  \Rightarrow (\exists\, alg_g \in Alg: alg_g \preceq alg_2)\,]
% \label{eq:integrityAlg}
% \end{gather}
% i.e.\ for each action that may be performed in the agent system, all
% dependent algorithms (or their specializations) must be available (i.e.\
% must be present in $Alg$).

The following function family is used by an agent of type $\tp$ to choose the
action to be executed:
\begin{equation}
\{ \omega^{\tp} : X \rightarrow \M(ACT) \}
\label{eq:omega}
\end{equation}
The choice of the action is thus based on the current state of the system
and is defined in stochastic terms. Usually only small part of the system
state will be taken into consideration (e.g.\ the agent's data or it's
aggregate's data).  Function $\omega$ allows an agent to choose only the
actions with compatible (the same or descendant) type:
\begin{gather}
\forall ag \in AG : ag=\tuple{id,\tp_1,dat_1,\ldots,dat_n}, \nonumber\\
\forall act \in ACT: act=\tuple{\tp_2,pre,post} \nonumber\\
\omega^{\tp}(x)(act) > 0 \iff \tp_1 \preceq \tp_2
\end{gather}
thus introducing a new type of agents requires adding a new function for
choosing the actions.


\subsubsection{Virtual multi-agent systems}

A crucial assumption of the model discussed here is that agents may be
organised in a tree-like structure of nested (multi-agent) subsystems
\citep{my:ICCS2009}.  It is realised so that an agent may provide an
environment for a group of other agents, which by themselves constitute a
multi-agent system. Thus agents which constitute inner nodes of this
structure may be perceived as \emph{aggregates} of other agents, but these
sub-agents constitute a complete multi-agent system according to
\eqref{eq:mas} -- essentially different then the one of the
\emph{aggregate} agent. In fact, the agents of different subsystems form a
structure, which is rather a collection of trees (a forest), which may be
perceived as a single tree with a ``virtual'' root node.

To identify an agent which provides the environment for a particular
multi-agent system a mapping is introduced:
\begin{equation}
\gamma: AS \rightarrow AG \cup \set{\varnothing}
\end{equation}
If a certain agent $ag\in Ag$ in $as=\tuple{Ag,Act}$ provides the
environment for $as^*=\tuple{Ag^*,Act^*}$ the mapping will give
$\gamma(as^*)=ag$, and this agent will be called an \emph{aggregate} for
$as^*$.  For a multi-agent system at the top of the hierarchy
$\gamma(as)=\varnothing$, since there is no real agent providing an
environment for this system (symbol $\varnothing$ may be perceived as
denoting a virtual root node of the hierarchy).

Thus the whole computational system consists of a set of agent systems
``linked'' according to the defined above $\gamma$ mapping. The state of
the computational system is a combination of the states of all the
subsystems and the current mapping defining their structure.  So the state
space may be described as:
\begin{align}
X   &= \tuple{2^{X_{AS}},\gamma}
\label{eq:state}
\end{align}
Actual state space will be constrained by the existence of agent types, and
the logical hierarchy of particular system, yet a more precise description of
the state space is beyond the scope of this paper.
% It is difficult to give a clear description of the state
% of the whole system, especially because we want to retain generality and
% do not try to model it's behavior in full extent.
% with following coherency condition fulfilled:
% \begin{gather}
% \forall \; as \in AS : \gamma(as) = \varnothing \nonumber\\
% \lor \; \gamma(as)=ag : \exists \; as^* =\tuple{Ag,Act} \in AS , ag \in Ag
% \end{gather}
% what means that every mas is either a top-level mas (has no parent) or
% is a child of another mas. 

% For a computational system consisting of a hierarchy of multi-agent
% (sub)systems one must reformulate functional integrity condistions. The
% system is functionally integral when the coherency conditions given by
% \eqref{eq:integrityAct} and \eqref{eq:integrityAlg} are true for all agent
% subsystems.

Considering queries it should be noted that they are functions of the whole
system state, but they are embedded in a particular agent system. The term
``embedded'' refers to the fact, that a certain query is located in an
agent system and it operates on the whole system state from that system's
point of view.  It often means that a query provides the information about
the agent's \emph{local} environment. In such a case the value of a query
depends only on the state of the agent system:
\begin{gather}
  \forall\,\chi=\tuple{\set{\ldots,as=\tuple{Ag,\ldots,qr_i,\ldots},\ldots},
    \gamma}\in X\nonumber\\
\lambda_i(\chi)=\lambda_i(Ag)
\end{gather}
or the state of the aggregate agent for this system:
\begin{equation}
  \forall\,\chi=\tuple{\set{\ldots,as,\ldots},\gamma}\in X
  \quad\lambda_i(\chi)=\lambda_i(\gamma(as))
\end{equation}
But of course queries may provide much more information, concerning other
agent systems at different levels of the structure. This way some
\emph{virtual} environment for an agent may by created, allowing to perform
observation of agents present in different agent systems. When supported by
appropriate actions, this in turn may allow to perform interactions (e.g.\
communication, migration) between different agent systems, which may be
together perceived as one \emph{virtual} multi-agent system.

A virtual multi-agent system is thus a way of perceiving a set of
\emph{cooperating} agent systems, in which the features physical structure
of the computation may be covered with accordingly defined queries and
actions. As a result some cooperation may arise between agents of different
systems, according to their relation in the hierarchy.  Actually the range
of possible interactions may be restricted, since agents of a virtual
multi-agent system perceive their environment through a dedicated set of
queries and actions, and may be unaware of the real physical structure of
the computation. In fact their cooperative behaviour may depend only on the
beliefs and intentions of agents that could be observed through their
virtual environments.

In a typical case, a virtual multi-agent system may be created by 
a set of ``neighbouring'' agent systems, i.e.\ systems, for which
their respective aggregate agents belong to one agent system:
\begin{equation}
  vAg = \bigcup_{as^*=\tuple{Ag^*,\ldots}\in vAs} Ag^*
\label{eq:vag}
\end{equation}
where:
\begin{gather}
  vAs=\set{as^*\,:\,\gamma(as^*)=\varnothing}\nonumber\\
  \lor\quad vAs=\set{as^*\,:\,\exists!\,Ag\;\gamma(as^*)\in Ag}
\label{eq:vas}  
\end{gather}

The concept of a virtual multi-agent system allows to define a computation
in the abstract way---e.g.\ independent of the actual hardware configuration.
This allows for better understanding of the system and for defining efficient
and scalable architectures.

%\begin{figure}
%\includegraphics[width=\textwidth]{mas.pdf}
%\caption{Physical and virtual structure of MAS}
%\label{fig:structure}
%\end{figure}

\subsubsection{Modelling island-based virtual multi-agent systems}
\label{sec:island}

Following the concept of a virtual multi-agent system as defined by
\eqref{eq:vag} and \eqref{eq:vas}, a simple two-level architecture may be
proposed, which will constitute a base for further considerations. This
model is an extracted and refactored part of EMAS model presented by the
authors \citep{my:ICCS2009}. The terminology of \emph{islands} and
\emph{individuals} comes from a classical coarse-grained (multiple-deme)
model of a parallel evolutionary algorithm \citep{Cantu-Paz}. The structure
consists of a system of agents-islands connected with a network of
communication channels, which are expressed in the model using ``neighbour''
addresses, and agents-individuals ``located'' on particular islands.

The model of an island-based virtual multi-agent system defines two types
of agents:
\begin{equation}
\TP=\{ ind, isl \}
\label{eq:types}
\end{equation}
where $ind$ denotes the type of an individual agent, which may perform some
computation or migrate among the islands, and $isl$ --- the type of
aggregate agent, which is introduced to manage subpopulations of individual
agents (an island).

Consequently, at the top of the hierarchical structure there is a system of
islands:
\begin{equation}
as=\tuple{Ag,\varnothing}\quad\gamma(as)=\varnothing
\label{eq:masemas}
\end{equation}
where:
\begin{equation}
Ag \ni ag=\tuple{id, isl, Nb}
\end{equation}
and $Nb \subset Ag$ is the set of neighbouring islands, which is used to
define migration topology.

Every island $ag$ provides the environment for a population of individual
agents:
\begin{equation}
\label{islandAS}
\forall \; ag \in Ag\;\;
\exists \; as^*=\tuple{Ag^*, Act^*, Alg^*, findLoc}: ag = \gamma(as^*)
\end{equation}
and an individual agent is defined as:
\begin{equation}
Ag^* \ni ag^*=\tuple{id, ind, sol}
\end{equation}
where:
\begin{description}
\item[$sol \in SOL$] represents the solution of the problem,
\item[$ACT \supseteq Act^* = \{comp, migr\}$] is the set of
  actions available in $as^*$:
  \begin{description}
	\item[$migr$] -- migration of an agent from one to another subpopulation,
	\item[$idle$] -- the action of doing nothing (agent does not change anything in the system),
  \end{description}
\item[$ALG \supseteq Alg^* = \{trans\} $] is the
  set of algorithms available in $as^*$,
\item[$findLoc=\mathcal{M}(AG)$] is the query which allows to choose the
  neighbouring island (using $Nb \subset Ag$) -- in fact, this query
  provides individual agents with the information about their local
  environment in a virtual multi-agent system.
\end{description}

Action of $idle$ performed by $ag^*=\tuple{id, ind, sol} \in Ag^*_1$ is
defined as follows:
\begin{equation}
Act \ni migr=\tuple{ind, pre, post}
\end{equation}
where:
\begin{gather}
pre = true \nonumber
\end{gather}
\begin{gather}
post = [\chi'=\chi\in X]  \nonumber
\end{gather}
Agent may intentionally choose to refrain from taking any activities in a
certain moment, therefore performing this action does not change the state
of the system at all.

Action of migration $migr$ performed by $ag^* \in
Ag^*_1 : \exists \; as^*_1 =\tuple{Ag^*_1,Act^*, Alg^*,findLoc_1} \
\land \ \gamma(as^*_1)=ag_1$ which migrates from $ag_1=\tuple{id_1, isl,
  Nb_1}$ to $ag_2=\underline{findLoc_1}=\tuple{id_2, isl, Nb_2} : \exists
\; as^*_2 =\tuple{Ag^*_2,Act^*, Alg^*,findLoc_2} \ \land \\
\gamma(as^*_2)=ag_2$ ($ag_2$ is randomly chosen from all neighbours of
$ag_1$ with uniform distribution), $ag^*=\tuple{id, ind, sol, en}$.

\begin{equation}
Act \ni migr=\tuple{ind, pre, post}
\end{equation}
where:
\begin{gather}
pre = [Nb_1\neq\varnothing] \nonumber
\end{gather}
\begin{gather}
  post = [en_1 > e_{migr} \Rightarrow\nonumber\\ Ag^*_1{'}=Ag^*_1 \setminus \{ag^*_1\}
  \land Ag^*_2{'}=Ag^*_2 \cup \{ag^*_1\}] \nonumber
\end{gather}
This action may be performed by an individual agent, located in the system
with at least one ``neighbouring'' island.  The agent leaves one island and
moves to another one. Thus this allows for the interaction between two
agent systems encompassed by a virtual multi-agent system.

% Several useful examples of such computation configurations follow (see Fig do narysowania):
% \begin{itemize}
% 	\item multi-deme evolutionary computation \citep{Cantu-Paz}: every environment is treated as evolutionary island
% 	and its inhabitants are provided with actions of migration, query for checking whether there is possibility
% 	of migrating to another environment and the data about neighboring environments ;
% 	\item evolutionary algorithm with population spread over multiple environments: instead of migration
% 	the query used for evaluation purposes may involve getting data from all neighboring environments,
% 	in this way the agents, though physically distant, may perceive that they work in one deme;
% 	\item hierarchical evolutionary algorithms \citep{hgs}: every environment is related to other 
% 	environment using additional relation coming from sprouting action, and may have its own
% 	sprouts, this information in its data.
% \end{itemize}

\subsubsection{Modelling an evolutionary multi-agent system}
\label{sec:emas}

The model of an evolutionary multi-agent system utilises the island-based
structure, as described in the previous section. Thus it defines two
analogous types of agents: $ind$ denotes the type of an individual agent,
and $isl$ --- the type of an island agent. The top-level system of
agents-island is defined as above.  Every island $ag$ provides the
environment for individual agents:
\begin{gather}
\forall \; ag \in Ag\;\;
\exists \; as^*=\tuple{Ag^*, Act^*, Alg^*, findAg, findLoc}:\nonumber\\
 ag = \gamma(as^*)
\end{gather}
and an individual agent is defined as:
\begin{equation}
Ag^* \ni ag^*=\tuple{id, ind, sol, en}
\end{equation}
where:
\begin{description}
\item[$sol \in SOL$] is the solution of the problem (usually for
  optimisation problems $SOL \subset \mathbb{R}^n, n\in \mathbb{N}$),
\item[$en \in \mathbb{R}^+$] is the amount of energy gathered by the
  individual agent,
\item[$ACT \supseteq Act^* = \{init, migr,get,repr,die,idle\}$] is the set of
  actions available in $as^*$:
  \begin{description}
	\item[$init$] -- initialisation of agent's solution,	
	\item[$get$] -- transfer of a portion of energy from one to another agent,
	\item[$repr$] -- creation of a new agent by two parents,
	\item[$die$] -- removing of an agent from the system,
  \end{description}
\item[$ALG \supseteq Alg^* = \{rand, prep, eval, recomb, mut, fitn\} $] is the
  set of algorithms available in $as^*$,
\item[$findAg=\mathcal{M}(AG)$] is the query which allows to
  choose the neighbouring individual agent (another agent present in the
  same system),
\item[$findLoc$] is the query as defined in the previous section.
\end{description}

An action of solution initialisation $init$ performed by $ag^*=\tuple{id,
  ind, sol, en} \in Ag^*$ is defined in the following way:
\begin{equation}
Act^* \ni init = \tuple{ind, [\tau(sol) = 0], [\tau(sol) = 1]}
\end{equation}
where $\tau : SOL \rightarrow \{0,1\}$ is a problem-dependent function,
which indicates if a solution is initialised (by returning 1) or not (by
returning 0).
% During this process a problem-dependent algorithm $prep \in Alg^*$ is used,
% and therefore: $init \leadsto prep$.  Also, algorithm $prep$ depends on
% another algorithm $rand$, necessary for generating random solutions. This
% is denoted as: $prep \leadsto rand$.

Action of energy transfer $get$ performed by $ag^*_1 \in Ag^*$, which meets
$ag^*_2=\underline{findAg}=\tuple{id_2, ind, sol_2, en_2} \in Ag^*$
(randomly chosen with uniform distribution from its neighbours),
$ag^*_1=\tuple{id_1, ind,  sol_1, en_1}$,
 may be
defined in the following way:
\begin{equation}
Act \ni get=\tuple{ind, pre, post}
\end{equation}
where:
$$pre = \# Ag^* > 1$$
\begin{gather}
  post = (\varphi(sol_1) < \varphi(sol_2) \Rightarrow\nonumber\\
   en_1' = en_1+e_{get}
  \land \  en_2' = en_2-e_{get}) \nonumber\\
  \lor \ (\varphi(sol_1) > \varphi(sol_2) \Rightarrow\nonumber\\
    en_1' = en_1-e_{get}
  \land \  en_2' = en_2+e_{get}	)\nonumber
	\end{gather}
where: $\varphi : SOL \rightarrow \mathbb{R}$ is the fitness function used
for the evaluation of solutions, the precise definition of this function is
problem-dependent.  $en_1'$ denotes the value of $en_1$ after performing
the action\footnote{Here and later the symbol $a'$ will denote the value of
  $a$ after performing the action (usually $a$ is used in precondition and
  $a'$ only in postcondition). This is similar to $old$ operator used in
  contract specification in Eiffel programming language \cite{meyer}.},
$\underline{A}(B)$ denotes the result of the random choice of the value from
the set $B$ with distribution $A$.\\	
This action may be performed by an individual agent, which has at least one
neighbour (agent in the same MAS subsystem).  Depending on the quality of
its solution, a part of energy is transferred from the worse to the better
agent.

% The action of energy transfer $get$ is performed by an
% individual agent depending on the quality of its solution, which is given
% by problem-dependent algorithm $eval$.  This relation may be defined as:
% $get \leadsto eval$. Moreover, evaluation requires existing of predefined
% fitness function implemented by algorithm $fitn$, therefore $eval \leadsto fitn$



Action of reproduction $repr$ performed by $ag^*_1 \in Ag^*$, which meets $ag^*_2=\tuple{id_2, ind, sol_2,
  en_2} \in Ag^*$ (randomly chosen with uniform distribution from its
neighbours),$ag^*_1=\tuple{id_1, ind,  sol_1, en_1}$ and produces the offspring agent\\ $ag^*_3=\tuple{id_3,
  ind, sol_3, en_3} \in Ag^*$ may be defined in the following way:
\begin{equation}
Act \ni repr=\tuple{ind, pre, post}
\end{equation}
where:
$$
pre = \# Ag^* > 1
$$
\begin{gather}
post =  en_1>e_{repr} \land \ en_2>e_{repr} \Rightarrow Ag^*{'} = Ag^* \cup \{ag^*_3\} \nonumber\\
\land \ en_3 = e_{0} \land \ en_1{'} = en_1 -\frac{1}{2}e_{0} \land \ en_2{'} = en_2-\frac{1}{2}e_{0}\nonumber\\ \land sol_3=\underline{\chi}(sol_1,sol_2)\nonumber
\end{gather}
where: $\chi : SOL \times SOL \rightarrow \mathcal{M}(SOL)$ is a variation
operator (recombination and mutation), its precise definition is
problem-dependent.\\ 
This action may be performed by an individual agent with at least one
neighbour, both with sufficient energy.  They create a new agent based on
their solutions.

% The action of reproduction $repr$ depends
% on the algorithms realizing recombination and mutation operators ---
% $recomb$ and $mut$ respectively. This
% is denoted as: $repr \leadsto recomb$, $repr \leadsto mut$.

Action of death $die$ performed by $ag^*=\tuple{id, ind, sol, en} \in Ag^*$ may be defined in the following way:
\begin{equation}
Act \ni die=\tuple{ind, pre, post}
\end{equation}
where:
$$pre = (en==0)$$
$$
post = (Ag^*{'} = Ag^* \setminus \{ag^*\})
$$
This action may be performed by an individual agent whose energy level
falls to zero.  This agent is removed from the system.

%Agents contained in MAS subsystems constitute a VMAS. 
%\begin{equation}
%VMAS = \{ \bigcup_i Ag^*_i : \exists \; mas^*_i=\tuple{Ag^*_i,Act^*_i}, \forall_i \; \gamma(mas^*_i) \in Ag \}
%\end{equation}
%where $Ag$ is the set of evolutionary islands defined in the formula \ref{eq:masemas}.



\subsection{EMAS concept and model summary}
The presented EMAS concept turned out to be an effective technique for optimisation of different problems,
moreover predefined formal models become a basis for proving, that EMAS is an universal optimiser \cite{fi1,fi2,bull}.
The model presented here makes possible easy identification of different pre- and post-conditions and identify so called
functional integrity conditions, that may affect the way of implementation:
\begin{itemize}
	\item pre- and post-conditions clauses in Design By Contract-like implementations \cite{meyer} may be easily constructed,
	\item requirements for series of unit tests may be identified (when considering object oriented, agile approaches),
	\item guarding clauses for functions expressed by actors (when considering functional approaches, like Erlang).
\end{itemize}


